Optimal Sketching for Kronecker Product Regression and Low Rank Approximation

We study the Kronecker product regression problem, in which the design matrix is a Kronecker product of two or more matrices. Given $A_i \in \mathbb{R}^{n_i \times d_i}$ for $i=1,2,\dots,q$ where $n_i \gg d_i$ for each $i$, and $b \in \mathbb{R}^{n_1 n_2 \cdots n_q}$, let $\mathcal{A} = A_1 \otimes A_2 \otimes \cdots \otimes A_q$. Then for $p \in [1,2]$, the goal is to find $x \in \mathbb{R}^{d_1 \cdots d_q}$ that approximately minimizes $\|\mathcal{A}x - b\|_p$. Recently, Diao, Song, Sun, and Woodruff (AISTATS, 2018) gave an algorithm which is faster than forming the Kronecker product $\mathcal{A}$ Specifically, for $p=2$ their running time is $O(\sum_{i=1}^q \text{nnz}(A_i) + \text{nnz}(b))$, where nnz$(A_i)$ is the number of non-zero entries in $A_i$. Note that nnz$(b)$ can be as large as $n_1 \cdots n_q$. For $p=1,$ $q=2$ and $n_1 = n_2$, they achieve a worse bound of $O(n_1^{3/2} \text{poly}(d_1d_2) + \text{nnz}(b))$. In this work, we provide significantly faster algorithms. For $p=2$, our running time is $O(\sum_{i=1}^q \text{nnz}(A_i) )$, which has no dependence on nnz$(b)$. For $p<2$, our running time is $O(\sum_{i=1}^q \text{nnz}(A_i) + \text{nnz}(b))$, which matches the prior best running time for $p=2$. We also consider the related all-pairs regression problem, where given $A \in \mathbb{R}^{n \times d}, b \in \mathbb{R}^n$, we want to solve $\min_{x} \|\bar{A}x - \bar{b}\|_p$, where $\bar{A} \in \mathbb{R}^{n^2 \times d}, \bar{b} \in \mathbb{R}^{n^2}$ consist of all pairwise differences of the rows of $A,b$. We give an $O(\text{nnz}(A))$ time algorithm for $p \in[1,2]$, improving the $\Omega(n^2)$ time needed to form $\bar{A}$. Finally, we initiate the study of Kronecker product low rank and low $t$-rank approximation. For input $\mathcal{A}$ as above, we give $O(\sum_{i=1}^q \text{nnz}(A_i))$ time algorithms, which is much faster than computing $\mathcal{A}$.

==> libtheorems.tex <==
% Code for theorems in multiple places
% Originally by Eric Price, placed in the public domain
%
% This lets you write the statement of a theorem/lemma in one place
% and insert it in multiple parts of a document.  This lets you
% include the statement of Lemma 3.2 in both the introduction and the
% place that it's proven, and the numbering can refer to the place
% where it's proven.
%
% Usage:
%
%  \define[optional title]{thm:main}{Theorem}{We show \[ x^2 + y^2 \geq 2xy \].}
%     Before you use it.
%
%  \state{thm:main}
%     in the place where you want the label to be generated
%
%  \restate{thm:main}
%     elsewhere.
%
%  To have consistent equation labels, use $\thmlabel{eq:1}$ rather
%  than $\label{eq:1}$.
%
%
%%%%% Begin code
\usepackage{etoolbox}

\makeatletter

% Define the various variables to be used in \state/\restate
\newcommand{\define}[4][ignore]{%
  \ifstrequal{#1}{ignore}{}{
  \@namedef{thmtitle@#2}{#1}}%
  \@namedef{thm@#2}{#4}%
  \@namedef{thmtypen@#2}{lemma}%
  \newtheorem{thmtype@#2}[theorem]{#3}%
  \newtheorem*{thmtypealt@#2}{#3~\ref{#2}}%
}

% State the theorem, generating the proper number.
\newcommand{\state}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
  \begin{thmtype@#1}
    }{
  \begin{thmtype@#1}[\@nameuse{thmtitle@#1}]
  }
    \label{#1}
    \@nameuse{thm@#1}
  \end{thmtype@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% Include the theorem, with the original numbering
\newcommand{\restate}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
    \begin{thmtypealt@#1}
    }{
  \begin{thmtypealt@#1}[\@nameuse{thmtitle@#1}]
  }
    \@nameuse{thm@#1}
  \end{thmtypealt@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

% For equations, this generates a new number if this is the first time
% the theorem is included, and reuses the old number otherwise.
\newcommand{\thmlabel}[1]{
  \@ifundefined{thmdone@\@nameuse{curthm}}{\label{#1}
    }{\tag*{\eqref{#1}}}
}
\makeatother
%%%%% End code


==> scrap.tex <==

\begin{algorithm*}[!t]\caption{Algorithm to $\ell_p$ sample $\Omega(r_2)$ entires of $\rho = (A_1 \otimes \cdots \otimes A_q)x'-b$}\label{alg:residualsample}
	\begin{algorithmic}[1]
		\Procedure{Residual $\ell_p$ sample}{$\rho, r_2$} %\Comment{Theorem~\ref{thm:l2_Kronregression}}
		\State Generate i.i.d. $p$-stable row-vectors $Z^{1}, Z^{2,j},\dots, Z^{q,j} \in \R^n$ for $j=1,2,\cdots \tau$ for $\tau = \Theta(\log(n))$.
		\State $r_3 \leftarrow \Theta(r_2 \log^{q^2}(n))$.
		\State Pre-compute  and store $Z^{i,j}A_i \in \R^{1 \times d_i}$ for all $i \in [q]$ and $j \in [\tau]$.
		\State $T_i \leftarrow \emptyset$ for $i \in [q]$. 
		\State $S \leftarrow \emptyset$ \Comment{$S$ a multi-set of tuples}
		
		\State $v_1^j \leftarrow \left( (\mathbb{I}_{n_1}) \otimes  (\bigotimes_{k = 2}^{q} Z^{k,j}) \rho\right) \in \R^{n_1}$ \Comment{$\mathbb{I}_n \in \R^{n \times n}$ is identity}
			\State Define $v_1 \in \R^{n_1}$ by $(v_1)_l = \median_{j \in [\tau]} \{		|(v_1^j)_l|\}$ for $l \in [n_1]$
		
			
		\For{$j = 1,2,\dots,r_3$}
		\State Sample $j^* \in [n_1]$ from the distribution $\left(\frac{|(v_1)_1|^p}{\|v_1\|_p^p}, \frac{|(v_1)_2|^p}{\|v_1\|_p^p}, \dots, \frac{|(v_1)_{n_1}|^p}{\|v_1\|_p^p}\right)$
		\State $S \leftarrow S \bigsqcup \{(j^*)\}$ \Comment{multi-set union}
		\State $T_1 \leftarrow T_1 \cup \{j^*\}$ \Comment{set union}
		\EndFor 
		\State Define $w(j) =  $
		
		\For{$i=2,\dots,q$}
		\For{ $j \in [\tau]$}
		\State $v_i^j \leftarrow \left( (\bigotimes_{k = 1}^{i-1} (Z^{k,j})_{T_{k}})) \otimes (\mathbb{I}_{n_i}) \otimes  (\bigotimes_{k = i+1}^{q} Z^{k,j}) \rho\right) \in \R^{n_i}$ 
		\EndFor
		\State Define $v_i \in \R^{n_i}$ by $(v_i)_l = \median_{j \in [\tau]} \{		|(v_i^j)_l|\}$ for $l \in [n_i]$
	
		\While{ There exists a $\vec{a} \in S$ without an index in the $i$-th coordinate}
		
		\State Sample $j^* \in [n_i]$ from the distribution $$\left(\frac{|(v_i)_1|^p}{\|v_i\|_p^p}, \frac{|(v_i)_2|^p}{\|v_i\|_p^p}, \dots, \frac{|(v_i)_{n_i}|^p}{\|v_i\|_p^p}\right)$$
			\For{each sample $\vec{a} = (a_{1}, a_{2}, \dots, a_{i-1}) \in S$} 
		\State $u_{\vec{a}}^j(j^*) =  \left((\bigotimes_{k = 1}^{i-1} e_{a_k}^\top) \otimes (e_{j^*}^\top) \otimes  (\bigotimes_{k = i+1}^{q} Z^{k,j}) \rho \right)$
		\State $u_{\vec{a}}(j^*) \leftarrow \median_{j \in [\tau]} \{	|u_{\vec{a}}^j|\}$.
		\EndFor
		\For{each $\vec{a} \in S$ without an $i$-th coordinate}
		\State sample $\vec{a} = (a_{1}, a_{2}, \dots, a_{i-1}) \in S$ with prob. $|u_{\vec{a}}(j^*)|^p/|(v_i)_{j^*}|^p$.
		\If{ $\vec{a} \in S$ is sampled}
		\State If $\vec{a} = (a_1,\dots, a_i)$ already has an $i$-th coordinate, do nothing.
		\State Otherwise, $\vec{a} = (a_1,\dots a_{i-1})$, and set $\vec{a} \leftarrow (a_1,\dots a_{i-1},j^*)$.
		\EndIf
		\EndFor
			\State Otherwise, with prob. $1-\sum_{\vec{a'} \in S}|u_{\vec{a'}}(j^*)|^p/|(v_i)_{j^*}|^p$, reject the sample $j^*$. 
		\EndWhile
		\State $T_i \leftarrow \{j \in [n_i]\; | \; \vec{a}_i = j \text{ for some } \vec{a} \in S  \}$
		\EndFor
		
		\State Let $v = \median_{j \in [\tau]} \left(|\bigotimes_{k=1}^q Z^{k,j}\rho|^p\right)$
		\For{each $\vec{a} \in S$}
		\State Compute probability $\gamma(\vec{a})$ that $\vec{a}$ was sampled above. 
		\State Remove $\vec{a}$ from $S$ with probability $(1/\gamma(\vec{a})) (  \kappa |\rho_{\vec{a}}|^p/ v)$ where $\kappa = \Theta(\log^{-q^2}(n))$. 
		\EndFor
		\State \Return Sample set $S$.
		
		\EndProcedure
	\end{algorithmic}
\end{algorithm*}
